A Spark of Vision-Language Intelligence: 2-Dimensional Autoregressive Transformer for Efficient Finegrained Image Generation

This work tackles the information loss bottleneck of vector-quantization (VQ) autoregressive image generation by introducing a novel model architecture called the 2-Dimensional Autoregression (DnD) Transformer. The DnD-Transformer predicts more codes for an image by introducing a new autoregression direction, \textit{model depth}, along with the sequence length direction. Compared to traditional 1D autoregression and previous work utilizing similar 2D image decomposition such as RQ-Transformer, the DnD-Transformer is an end-to-end model that can generate higher quality images with the same backbone model size and sequence length, opening a new optimization perspective for autoregressive image generation. Furthermore, our experiments reveal that the DnD-Transformer's potential extends beyond generating natural images. It can even generate images with rich text and graphical elements in a self-supervised manner, demonstrating an understanding of these combined modalities. This has not been previously demonstrated for popular vision generative models such as diffusion models, showing a spark of vision-language intelligence when trained solely on images. Code, datasets and models are open at https://github.com/chenllliang/DnD-Transformer.

==> contents/findings.tex <==
\subsection{Sampling Trend Difference Between 1D-AR and DnD}

\subsection{Multiple Prediction Heads' Loss Decomposition}

==> contents/limitation.tex <==
While these initial findings are encouraging, further investigation is warranted given the constraints of this study, including limited resources and the publication's page restrictions.

\subsection{Better Multi-layer Discrete Representation for Image}

\subsection{Conditional Rich-Text Generation}

\subsection{Knowledge Transfer from Large Language Models}

==> table/PPLocr.tex <==






















==> table/rqvae_rocr.tex <==

\begin{table}[ht]
\centering
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\textbf{Method} & \textbf{Data} & \textbf{Epoch} & \textbf{R-1 P} & \textbf{R-1 R} & \textbf{R-1 F1} & \textbf{R-2 P} & \textbf{R-2 R} & \textbf{R-2 F1} & \textbf{R-L P} & \textbf{R} & \textbf{R-L F1} \\ \hline
RQVAE & ImageNet &  & 0.05 & 0.01 & 0.01 & 0.03 & 0.01 & 0.01 & 0.05 & 0.01 & 0.01 \\ \hline
RQVAE & ImageNet + PDF & 10 & 37.57 & 40.85 & 31.70 & 25.54 & 27.70 & 22.10 & 34.87 & 37.96 & 29.48 \\ \hline
RQVAE & ImageNet + PDF & 15 & 43.91 & 46.20 & 38.32 & 31.74 & 33.38 & 28.17 & 41.18 & 43.44 & 36.05 \\ \hline
RQVAE & ImageNet + PDF & 20 & 42.56 & 45.24 & 37.50 & 31.23 & 33.23 & 28.05 & 40.31 & 42.58 & 35.48 \\ \hline
RQVAE & ImageNet + PDF & 25 & 47.02 & 48.94 & 41.87 & 36.20 & 37.11 & 32.73 & 44.48 & 46.38 & 39.77 \\ \hline
RQVAE & ImageNet + PDF & 30 & 45.71 & 49.59 & 40.99 & 35.79 & 38.03 & 32.52 & 43.25 & 46.99 & 38.95 \\ \hline
RQVAE & ImageNet + PDF & 35 & 47.82 & 49.15 & 41.69 & 37.44 & 37.53 & 33.04 & 45.01 & 46.27 & 39.29 \\ \hline
RQVAE & ImageNet + PDF & 40 & 50.50 & 49.56 & 43.52 & 39.42 & 38.15 & 34.63 & 47.93 & 47.09 & 41.40 \\ \hline
RQVAE & ImageNet + PDF & 45 & 45.45 & 47.64 & 38.88 & 35.20 & 36.03 & 30.77 & 42.80 & 45.08 & 36.78 \\ \hline
\end{tabular}
\caption{Results for RQVAE on ImageNet and ImageNet+PDF}
\label{table:results}
\end{table}

